Turbulent boundary layer with strong favorable pressure gradient and curvature effects: Streamline coordinate and scaling analysis

Direct numerical simulation (DNS) of a turbulent boundary layer over the Gaussian (Boeing) bump is performed. This boundary layer exhibits a series of adverse and favorable pressure gradients and convex and concave curvature effects before separating. These effects on turbulent boundary layers are characterized and compared to a lower Reynolds number flow over the same geometry. The momentum budgets are analyzed in the streamline-aligned coordinate system upstream of the separation region. These momentum budgets allow the simplification of equations to facilitate an integral analysis. Integral analysis-based scalings for Reynolds stresses in the inner and outer regions of the boundary layer are also formulated. These proposed scalings exhibit a better collapse of Reynolds stress profiles compared to friction velocity scaling and Zagarola-Smits scaling in the strong favorable pressure gradient region and in the mild adverse pressure region that precedes it in this flow.

==> TKEDiscussion.tex <==
\section{Appendix B: Turbulent kinetic energy budget}

Analysis of the turbulent kinetic energy budget involves understanding and interpreting the balance between different terms of the turbulent kinetic energy equation:

\begin{multline}
     \underbrace{\frac{\p k}{\p t}}_{\text{Acceleration}} + \underbrace{\bar{u}_i \frac{\p k}{\p x_i}}_{\text{Advection}} = \underbrace{- \overline{u'_i u'_j} \frac{\p \bar{u}_i}{\p x_j}}_{\text{Production}} - \underbrace{ \frac{\p \overline{u'_i u'_i u'_j}}{\p x_j}}_{\substack{\text{Turbulent}\\ \text{Transport}}} - \underbrace{
    \frac{1}{\rho} \frac{ \p \overline{u'_i p'}}{\p x_i}}_{\substack{\text{Pressure}\\ \text{Diffusion}}} + \underbrace{2 \nu \frac{\p \overline{u'_j S'_{ij}}}{\p x_i}}_{\substack{\text{Velocity}\\ \text{Strain}}} - \underbrace{ 2 \nu \overline{S'_{ij} S'_{ij}}}_{\text{Dissipation}}
\end{multline}

\noindent where $S'_{ij} = \frac{1}{2} \Big( \frac{\p u'_i}{\p x_j} + \frac{\p u'_j}{\p x_i}\Big)$ is the strain-rate fluctuation arising from Reynolds decomposition.

\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.32\textwidth]{Figures/TKE_Budget/Budget_localutau_xLm0p45.png}}
    \subfigure{\includegraphics[width=0.32\textwidth]{Figures/TKE_Budget/Budget_localutau_xLm0p39.png}}
    \subfigure{\includegraphics[width=0.32\textwidth]{Figures/TKE_Budget/Budget_localutau_xLm0p29.png}}    
    
    \subfigure{\includegraphics[width=0.32\textwidth]{Figures/TKE_Budget/Budget_localutau_xLm0p15.png}}
    \subfigure{\includegraphics[width=0.32\textwidth]{Figures/TKE_Budget/Budget_localutau_xLm0p079.png}}
    \subfigure{\includegraphics[width=0.32\textwidth]{Figures/TKE_Budget/Budget_localutau_xLm0p006.png}}    
    \caption{TKE budget terms at several $x/L$ stations. The colors denote different TKE budget terms: }
    \label{fig:TKE_Budget_xLloc}
\end{figure}

Turbulent kinetic energy (TKE) budget terms at several $x/L$ locations are shown in \figref{TKE_Budget_xLloc}. We observe that each term in the turbulent kinetic energy budget qualitatively behaves similar at several $x/L$ locations. This behavior implies that pressure gradient effects, internal layers and curvature effects do not significantly affect the distribution between different terms. The most significant differences are observed for the TKE production and TKE dissipation. 

\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.49\textwidth]{Figures/TKE_Budget/Prod_localutau_XLcomp_APG.png}}
    \subfigure{\includegraphics[width=0.49\textwidth]{Figures/TKE_Budget/Prod_localdelta_XLcomp_APG.png}}
    
    \caption{Production of turbulent kinetic energy scaled (a) in inner-region units and (b) in outer-region units for APG region at several $x/L$ stations. The colors denote different TKE budget terms: }
    \label{fig:Prod_scale_APG}
\end{figure}

\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.49\textwidth]{Figures/TKE_Budget/Prod_localutau_XLcomp_FPG.png}}
    \subfigure{\includegraphics[width=0.49\textwidth]{Figures/TKE_Budget/Prod_localdelta_XLcomp_FPG.png}}
    ßß
    \caption{Production of turbulent kinetic energy scaled (a) in inner-region units and (b) in outer-region units for FPG region at several $x/L$ stations. }
    \label{fig:Prod_scale_FPG}
\end{figure}

Production of turbulent kinetic energy in \figref{Prod_scale_APG} shows significantly different behavior in the APG region when presented with inner-region and outer-region scaling. In the APG region, we observe slight differences in the peak production across $x/L$ stations when expressed in inner-region units. When expressed in outer-region units, we observe that peak production moves to a lower $n/\delta$ indicating the peak production moves closer to the wall relative to the boundary layer thickness in the presence of APG. However, the position of the production peak does not change relative to the viscous length-scale in the APG region. The growth of the boundary layer downstream does not imply a similar shift of the production peak as turbulent kinetic energy production is dominant in the inner region of the boundary layer and scales with inner region units. We also observe that the peak production decreases significantly in the APG region when scaled by outer-region units further enforcing the idea that production scales based on the inner region of the boundary layer. 

Production of turbulent kinetic energy in \figref{Prod_scale_FPG} shows significantly different behavior in the FPG region when presented with  inner-region and outer-region scaling. When production is scaled in inner region units, we observe a shift of the location of peak production away from the wall as the FPG increases until $x/L \leq -0.1$ and then a shift of the profile closer to the wall as the FPG decreases for $-0.1 \leq x/L \leq 0$. When the production is scaled in outer region units, we observe a shift of production peak towards the wall for the entire FPG region. As shown in \figref{BLThick}, the boundary layer thickness reduces in the FPG region. These results indicate that the production peak moves closer to the wall faster than the decreasing boundary layer thickness. A decrease in the production in the outer region of the boundary layer is also observed as we move downstream in the FPG region. This decrease is a result of stabilizing effect of pressure gradient and streamline curvatures on turbulence production. 

\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.49\textwidth]{Figures/TKE_Budget/Dissip_localutau_XLcomp_APG.png}}
    \subfigure{\includegraphics[width=0.49\textwidth]{Figures/TKE_Budget/Dissip_localdelta_XLcomp_APG.png}}
    
    \caption{Dissipation of turbulent kinetic energy scaled (a) in inner-region units and (b) in outer-region units for APG region at several $x/L$ stations. }
    \label{fig:Dissip_scale_APG}
\end{figure}

\begin{figure}
    \centering
    \subfigure{\includegraphics[width=0.49\textwidth]{Figures/TKE_Budget/Dissip_localutau_XLcomp_FPG.png}}
    \subfigure{\includegraphics[width=0.49\textwidth]{Figures/TKE_Budget/Dissip_localdelta_XLcomp_FPG.png}}
    
    \caption{Dissipation of turbulent kinetic energy scaled (a) in inner-region units and (b) in outer-region units for FPG region at several $x/L$ stations. }
    \label{fig:Dissip_scale_FPG}
\end{figure}

Dissipation of turbulent kinetic energy is the APG and FPG regions of the flow are shown in \figref{Dissip_scale_APG} and \figref{Dissip_scale_FPG} respectively. Previous studies \cite{} on turbulent boundary layer in strong APG indicate the presence of a secondary peak for TKE production and dissipation. Such a behavior is not observed in the DNS which further assures that that the flow exhibits only mild APG effects. For the FPG region, scaled dissipation decreases in the outer region indicating the stabilizing influence of pressure gradient in that region. 

\section{Acknowledgements}

The authors would like to acknowledge the Transformational Tools and Technologies Project of the National Aeronautics and Space Administration (NASA) 80NSSC18M0147 for funding of this work. Moreover, this research used computational resources of the NASA High-End Computing (HEC) Program through the NASA Advanced Supercomputing (NAS) Division at Ames Research Center as well as the Argonne Leadership Computing Facility which is a DOE Office of Science User Facility supported under Contract DE-AC02-06CH11357. Finally, the authors would like to thank Dr. Ali Uzun for providing reference DNS data for comparison. We thank Dr.\@ Christopher Rumsey and Dr.\@ Philippe Spalart for insightful discussions and comments. 
